The Origin of Massive O-type Field Stars. Part I: A Search for Clusters

We present a study aimed at clarifying the birthplace for 43 massive O-type field stars. In this first paper we present the observational part: a search for stellar clusters near the target stars. We derive stellar density maps at two different resolving scales, viz. 0.25pc and 1.0pc from NTT and TNG imaging and the 2MASS catalogue. These scales are typical for cluster sizes. The main result is that the large majority of the O-type field population are isolated stars: only 12% (5 out of 43) of the O-type field stars is found to harbour a small-scale stellar cluster. We review the literature and aim at characterizing the stellar field of each O-type field star with the emphasis on star formation and the presence of known young stellar clusters. An analysis of the result of this paper and a discussion of the O-type field population as products of a dynamical ejection event is presented in an accompanying paper.

==> FIG_TEX/Fig10.tex <==
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd123056_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd123056_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd123056_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd124314_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd124314_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd124314_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd125206_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd125206_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd125206_sden.eps}
\caption[]{As in Fig.\,\ref{f_hd3687} for stars HD\,123056, HD\,124314, and HD\,125206.}
\label{f_hd1252}
\end{figure*}


==> FIG_TEX/Fig11.tex <==
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd135240_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd135240_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd135240_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd135591_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd135591_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd135591_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd153426_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd153426_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd153426_sden.eps}
\caption[]{As in Fig.\,\ref{f_hd3687} for stars HD\,135240, HD\,135591, and HD\,153426.}
\label{f_hd1534}
\end{figure*}


==> FIG_TEX/Fig12.tex <==
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd153919_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd153919_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd153919_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd154368_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd154368_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd154368_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd154643_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd154643_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd154643_sden.eps}
\caption[]{As in Fig.\,\ref{f_hd3687} for stars HD\,153919, HD\,154368, and HD\,154643.}
\label{f_hd1546}
\end{figure*}




==> FIG_TEX/Fig13.tex <==
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd154811_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd154811_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd154811_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd158186_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd158186_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd158186_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd161853_23_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd161853_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd161853_sden.eps}
\caption[]{As in Fig.\,\ref{f_hd3687} for stars HD\,154811, HD\,158186, and HD\,161853.}
\label{f_hd1618}
\end{figure*}


==> FIG_TEX/Fig14.tex <==
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd163758_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd163758_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd163758_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd165319_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd165319_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd165319_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd169515_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd169515_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd169515_sden.eps}
\caption[]{As in Fig.\,\ref{f_hd3687} for stars HD\,163758, HD\,165319, and HD\,169515.}
\label{f_hd1695}
\end{figure*}


==> FIG_TEX/Fig15.tex <==

\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd175754_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd175754_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd175754_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd175876_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd175876_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd175876_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd188209_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/TNG/hd188209_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd188209_sden.eps}
\caption[]{As in Fig.\,\ref{f_hd3687} for stars HD\,175754, HD\,175876, and HD\,188209.}
\label{f_hd1882}
\end{figure*}



==> FIG_TEX/Fig16.tex <==

\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd193793_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/TNG/hd193793_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd193793_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd195592_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/TNG/hd195592_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd195592_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd201345_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/TNG/hd201345_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd201345_sden.eps}
\caption[]{As in Fig.\,\ref{f_hd3687} for stars HD\,193793, HD\,195592, and HD\,201345.}
\label{f_hd2013}
\end{figure*}


==> FIG_TEX/Fig17.tex <==
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd202124_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/TNG/hd202124_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd202124_sden.eps}
\caption[]{As in Fig.\,\ref{f_hd3687} for star HD\,202124.}
\label{f_hd2021}
\end{figure*}


==> FIG_TEX/Fig3.tex <==
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd1337_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/TNG/hd1337_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd1337_sden.eps}
\end{figure*}

\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd15137_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/TNG/hd15137_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd15137_sden.eps}
\end{figure*}

\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd36879_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd36879_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd36879_sden.eps}
 \caption[]{Left panels: $\rm K_{s}$-band image with 5 arcmin on a side.
 Middle panels: correspoding surface stellar density maps. Right panels:
 density maps derived from the 2MASS PSC, for stars HD\,1337, HD\,15137 and
 HD\,36879.  Ordinates are in arcmin for the middle and right panels. Contours are 1\vspace{0.05cm}$\sigma$ spaced deviations from
 the average stellar density value.}
\label{f_hd3687}
\end{figure*}


==> FIG_TEX/Fig4.tex <==
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd39680_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd39680_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd39680_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd41161_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/TNG/hd41161_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd41161_sden.eps}
\end{figure*}
\begin{figure*}
 \center
\includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd48279_ks.ps}
\includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd48279_sden.eps}
\includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd48279_sden.eps}
\caption[]{As in Fig.\,\ref{f_hd3687} for stars HD\,39680, HD\,41161, and HD\,48279.}
\label{f_hd4827}
\end{figure*}



==> FIG_TEX/Fig5.tex <==
\begin{figure*}[t,h]
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd52266_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd52266_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd52266_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd52533_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd52533_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd52533_sden.eps}
\end{figure*}
\begin{figure*}[t,h]
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd57682_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd57682_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd57682_sden.eps}
\caption[]{As in Fig.\,\ref{f_hd3687} for stars HD\,52266, HD\,52533, and HD\,57682.}
\label{f_hd5768}
\end{figure*}


==> FIG_TEX/Fig6.tex <==
\begin{figure*}[t,h]
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd60848_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd60848_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd60848_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd66811_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd66811_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd66811_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd75222_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd75222_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd75222_sden.eps}
\caption[]{As in Fig.\,\ref{f_hd3687} for stars HD\,60848, HD\,66811, and HD\,75222.}
\label{f_hd7522}
\end{figure*}



==> FIG_TEX/Fig7.tex <==
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd89137_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd89137_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd89137_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd91452_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd91452_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd91452_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd96917_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd96917_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd96917_sden.eps}
\caption[]{As in Fig.\,\ref{f_hd3687} for stars HD\,89137, HD\,91452, and HD\,96917.}
\label{f_hd9691}
\end{figure*}


==> FIG_TEX/Fig8.tex <==
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd105627_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd105627_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd105627_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd112244_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd112244_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd112244_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd113659_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd113659_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd113659_sden.eps}
\caption[]{As in Fig.\,\ref{f_hd3687} for stars HD\,105627, HD\,112244, and HD\,113659.}
\label{f_hd1136}
\end{figure*}


==> FIG_TEX/Fig9.tex <==
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd117856_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd117856_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd117856_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd120678_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd120678_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd120678_sden.eps}
\end{figure*}
\begin{figure*}
 \center
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/PS_IMAGES/hd122879_ks.ps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/Density_maps_new2/NTT/hd122879_sden.eps}
 \includegraphics[height=5cm,width=5cm,angle=-90]{Input/2MASS_density2/2mass_as_hd122879_sden.eps}
\caption[]{As in Fig.\,\ref{f_hd3687} for stars HD\,117856, HD\,120678, and HD\,122879.}
\label{f_hd1228}
\end{figure*}


==> STARS_TEX/hd48149.tex <==
\subsection{HD\,48149}
\label{visbi48}

According to SIMBAD, this is a G2/G3V star, followed by the extra note that
confusion exists between HD\,48149 and HD\,46149. The latter is an 08.5V star in
cluster NGC\,2244. We do not show the density maps of HD\,48149. 

% There is an unfortunate type-error in the M98 table and subsequently we
% imaged HD\,48149, the G2/G3V star.

